Swap Regret and Correlated Equilibria Beyond Normal-Form Games

Swap regret is a notion that has proven itself to be central to the study of general-sum normal-form games, with swap-regret minimization leading to convergence to the set of correlated equilibria and guaranteeing non-manipulability against a self-interested opponent. However, the situation for more general classes of games -- such as Bayesian games and extensive-form games -- is less clear-cut, with multiple candidate definitions for swap-regret but no known efficiently minimizable variant of swap regret that implies analogous non-manipulability guarantees. In this paper, we present a new variant of swap regret for polytope games that we call ``profile swap regret'', with the property that obtaining sublinear profile swap regret is both necessary and sufficient for any learning algorithm to be non-manipulable by an opponent (resolving an open problem of Mansour et al., 2022). Although we show profile swap regret is NP-hard to compute given a transcript of play, we show it is nonetheless possible to design efficient learning algorithms that guarantee at most $O(\sqrt{T})$ profile swap regret. Finally, we explore the correlated equilibrium notion induced by low-profile-swap-regret play, and demonstrate a gap between the set of outcomes that can be implemented by this learning process and the set of outcomes that can be implemented by a third-party mediator (in contrast to the situation in normal-form games).

==> preamble-ec.tex <==

%\usepackage{amssymb}
%\usepackage{amsmath}
%\usepackage{amsthm}
% \usepackage{fullpage}
\usepackage{latexsym}
\usepackage{graphicx}
\usepackage{color}
\usepackage{graphics}
%\usepackage[round]{natbib}
\bibliographystyle{plainnat}
\usepackage{cancel}
\usepackage{thm-restate}
\usepackage{mathtools}
\usepackage[mathscr]{euscript}
\usepackage{hyperref}
\usepackage{tikz,wrapfig}
%\usepackage{cleveref}

\usepackage{enumitem}

% \usepackage{fullpage}


%\usepackage{algorithmic}
\usepackage[algo2e,ruled]{algorithm2e}
\usepackage{algorithm}
\usepackage{algpseudocode}

% \newcommand\hmmax{0}
% \newcommand\bmmax{0}


% \let\vec\undefined
% \usepackage{MnSymbol}
% \DeclareMathAlphabet\mathbb{U}{msb}{m}{n}
% \usepackage{xpatch}

\def\Rset{\mathbb{R}}
\def\Sset{\mathbb{S}}

\let\Pr\undefined
\let\P\undefined
\DeclareMathOperator*{\Pr}{\mathbb{P}}
\DeclareMathOperator*{\P}{\mathbb{P}}
\DeclareMathOperator*{\E}{\mathbb E}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\esssup}{esssup}
\DeclareMathOperator*{\dom}{dom}
\DeclareMathOperator*{\cont}{cont}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\core}{core}
\DeclareMathOperator*{\pen}{pen}
\DeclareMathOperator{\VCdim}{VCdim}
\DeclareMathOperator{\Pdim}{Pdim}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\diag}{diag}


\DeclareMathOperator{\Ind}{\mathbb{I}} 

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert} 
\DeclarePairedDelimiter{\bracket}{[}{]}
\DeclarePairedDelimiter{\curl}{\{}{\}}
\DeclarePairedDelimiter{\norm}{\|}{\|}
\DeclarePairedDelimiter{\paren}{(}{)}
\DeclarePairedDelimiter{\tri}{\langle}{\rangle}
\DeclarePairedDelimiter{\dtri}{\llangle}{\rrangle}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}


\newcommand{\dest}{\mathrm{dest}}
\newcommand{\src}{\mathrm{src}}
\newcommand{\ilab}{\mathsf{ilab}}
\newcommand{\olab}{\mathsf{olab}}
\newcommand{\Ber}{\mathsf{Ber}}
\newcommand{\weight}{\mathsf{weight}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\sA}{{\mathscr A}}
\newcommand{\sB}{{\mathscr B}}
\newcommand{\sC}{{\mathscr C}}
\newcommand{\sD}{{\mathscr D}}
\newcommand{\sF}{{\mathscr F}}
\newcommand{\sG}{{\mathscr G}}
\newcommand{\sH}{{\mathscr H}}
\newcommand{\sI}{{\mathscr I}}
\newcommand{\sJ}{{\mathscr J}}
\newcommand{\sK}{{\mathscr K}}
\newcommand{\sL}{{\mathscr L}}
\newcommand{\sM}{{\mathscr M}}
\newcommand{\sP}{{\mathscr P}}
\newcommand{\sS}{{\mathscr S}}
\newcommand{\sT}{{\mathscr T}}
\newcommand{\sU}{{\mathscr U}}
\newcommand{\sX}{{\mathscr X}}
\newcommand{\sY}{{\mathscr Y}}
\newcommand{\sZ}{{\mathscr Z}}

\newcommand{\bA}{{\mathbf A}}
\newcommand{\bB}{{\mathbf B}}
\newcommand{\bD}{{\mathbf D}}
\newcommand{\bH}{{\mathbf H}}
\newcommand{\bK}{{\mathbf K}}
\newcommand{\bL}{{\mathbf L}}
\newcommand{\bM}{{\mathbf M}}
\newcommand{\bN}{{\mathbf N}}
\newcommand{\bP}{{\mathbf P}}
\newcommand{\bQ}{{\mathbf Q}}
\newcommand{\bR}{{\mathbf R}}
\newcommand{\bV}{{\mathbf V}}
\newcommand{\bW}{{\mathbf W}}
\newcommand{\bX}{{\mathbf X}}
\newcommand{\bY}{{\mathbf Y}}
\newcommand{\bZ}{{\mathbf Z}}
\newcommand{\bl}{{\mathbf l}}
\newcommand{\bx}{{\mathbf x}}
\newcommand{\by}{{\mathbf y}}
\newcommand{\br}{{\mathbf r}}
\newcommand{\blambda}{{\mathbf \lambda}}
\newcommand{\bu}{{\mathbf u}}
\newcommand{\bv}{{\mathbf v}}
\newcommand{\bw}{{\mathbf w}}
\newcommand{\bn}{{\mathbf n}}
\newcommand{\bp}{{\mathbf p}}



\newcommand{\sfp}{{\mathsf p}}
\newcommand{\sfq}{{\mathsf q}}
\newcommand{\sfr}{{\mathsf r}}
\newcommand{\sfE}{{\mathsf E}}
\newcommand{\sfB}{{\mathsf B}}
\newcommand{\sfD}{{\mathsf D}}
\newcommand{\sfS}{{\mathsf S}}
\newcommand{\sfT}{{\mathsf T}}

\newcommand{\mat}[1]{{\mathbf #1}}

\newcommand{\supcvstab}{\chi}
\newcommand{\avgcvstab}{\bar{\chi}}
\newcommand{\supdiam}{\Delta}
\newcommand{\maxdiam}{\Delta_{\max}}
\newcommand{\avgdiam}{\bar{\Delta}}
\newcommand{\swap}{{\sc swap}}
\newcommand{\ndfst}{{\sc NDFST}}

\newcommand{\R}{\mathfrak R}
\newcommand{\bsigma}{{\boldsymbol \sigma}}

\newcommand{\h}{\widehat}
\newcommand{\ov}{\overline}
\newcommand{\wt}{\widetilde}
\newcommand{\e}{\epsilon}
\newcommand{\eps}{\varepsilon}
\newcommand{\ignore}[1]{}

\newcommand{\wtu}{\widetilde{u}}
\newcommand{\wtO}{\widetilde{O}}

\newcommand{\yV}{y^{V}}
\newcommand{\xV}{x^{V}}
\newcommand{\byV}{\by^{V}}
\newcommand{\bxV}{\bx^{V}}

\DeclareMathOperator{\sgn}{\mathsf{sgn}}
\DeclareMathOperator{\BR}{\mathsf{BR}}
\DeclareMathOperator{\Stack}{\mathsf{Stack}}
\DeclareMathOperator{\Reg}{\mathsf{Reg}}
\DeclareMathOperator{\Swap}{\mathsf{SwapReg}}
\DeclareMathOperator{\SwapDist}{\mathsf{SwapDist}}
\DeclareMathOperator{\LinSwap}{\mathsf{LinSwapReg}}
\DeclareMathOperator{\CorrSwap}{\mathsf{ProfSwapReg}}
\DeclareMathOperator{\CorrDist}{\mathsf{ProfSwapDist}}
\DeclareMathOperator{\PolySwap}{\mathsf{PolySwapReg}}
\DeclareMathOperator{\NormSwap}{\mathsf{NFSwapReg}}
\DeclareMathOperator{\AppLoss}{\mathsf{AppLoss}}
\DeclareMathOperator{\Adv}{\mathsf{Adv}}
\DeclareMathOperator{\Unif}{\mathsf{Unif}}
\DeclareMathOperator{\Proj}{\mathrm{Proj}}
\DeclareMathOperator{\ShellProj}{\mathsf{ShellProj}}

\newcommand{\sr}{\ell}
\newcommand{\srset}{\cL}
\usepackage{comment}
% \newcommand\bmmax{0} % default 4
\usepackage{bm}

\usepackage{blkarray}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{question}{Question}

\newcommand{\optset}{\cY}
\newcommand{\learnset}{\cX}
\newcommand{\vset}{\cV}
\newcommand{\learnvert}{\vset(\learnset)}
\newcommand{\optvert}{\vset(\optset)}
\newcommand{\csp}{\phi}
\newcommand{\cspV}{\phi^{V}}
\newcommand{\ball}{\cB}

% \usepackage{thmtools}
% \usepackage{thm-restate}
% \declaretheorem{thm}


%\newcommand\jon[1]{{[\color{magenta}{\textbf{Jon:}~#1}]}}

\newcommand\jon[1]{}


%\newcommand\nat[1]{{[\color{blue}{\textbf{Natalie:}~#1}]}}


\newcommand\nat[1]{}


%\newcommand\esh[1]{{[\color{red}{\textbf{Eshwar:}~#1}]}}

\newcommand\esh[1]{}

%\newcommand\mm[1]{{[\color{orange}{\textbf{MM:}~#1}]}}

\newcommand\mm[1]{}




==> scratchpad.tex <==
#Annotating the nine coordinates 


# Convention -- 10 means the first coordinate is 1 and the second is 0
#More specifically, let us call player 1's action v1v2 and player 2's action w1w2 
#ECh vi/wi can take values in {0,1}
#All are sums 
# phi1  = v1w1 (i.e. 1 iff both v1 and w1 are 1) -bottom right 4 elements
#phi2 = v1w2  (intersection of bottom two rows and middle columns)
#phi3 = v1 (bottom two rows)
#phi4 = v2w1 (middle rows and right columns)
#phi5 = v2w2 (middle row and middle cols)
#phi6 = v2 (middle two rows)
#phi7 = w1 (right cols)
#phi8 = w2 ( middle cols)
#phi9 = 1
